Social Amplification Dominates Collective Hazard Response

Large-scale hazards affect societies not only through direct physical impacts but also through emotions that spread across populations. Fueled by social amplification and networked communication, collective emotions often diverge markedly from underlying physical threats, pressuring policymakers toward suboptimal decisions that erode long-term societal resilience and misalign risk governance priorities. Yet when exactly these collective emotions mirror hazard severity and when they are warped by social dynamics remains poorly understood. We introduce a compact, interpretable model that couples hazard exposure with networked emotional contagion and identifies the transition from proportionate responses to an amplification regime sustained by negativity bias. Applying this framework to the COVID-19 pandemic in the United States, we integrate state-level epidemiological data with large-scale stress signals inferred from Twitter/X activity. Our analysis shows that social influence outweighed direct hazard forcing in over 80\% of U.S. states during the study period, and that amplified stress covaries with major economic indices. These findings reveal a measurable regularity in societal hazard response, enabling quantitative anticipation of collective emotional tipping points and supporting community resilience under large-scale hazards.

==> latexmkrc <==
# Shared latexmk configuration for local builds and Overleaf.
#
# Overleaf only reads a project-level file named `latexmkrc` (no leading dot).
# The custom dependency below is adapted from Overleaf's official xr guidance:
# when SI.tex needs main.aux, latexmk will compile main.tex automatically and
# copy the generated aux file next to the source so xr can import the labels.

# Ensure SyncTeX data is generated for forward/inverse search.
$pdflatex = 'pdflatex -synctex=1 -interaction=nonstopmode -file-line-error %O %S';
$xelatex  = 'xelatex  -synctex=1 -interaction=nonstopmode -file-line-error %O %S';
$lualatex = 'lualatex -synctex=1 -interaction=nonstopmode -file-line-error %O %S';

$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();
push @sub_doc_options, '-pdf';  # Keep external documents on pdfLaTeX like the main build.

push @file_not_found, '^No file\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] ) {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
            rdb_add_generated( "$sub_doc_output/$base_name.aux" );
            copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
    }
    return 0;
}

1;

